DuET: Dual Execution for Test Output Prediction with Generated Code and Pseudocode

This work addresses test output prediction, a key challenge in test case generation. To improve the reliability of predicted outputs by LLMs, prior approaches generate code first to ground predictions. One grounding strategy is direct execution of generated code, but even minor errors can cause failures. To address this, we introduce LLM-based pseudocode execution, which grounds prediction on more error-resilient pseudocode and simulates execution via LLM reasoning. We further propose DuET, a dual-execution framework that combines both approaches by functional majority voting. Our analysis shows the two approaches are complementary in overcoming the limitations of direct execution suffering from code errors, and pseudocode reasoning from hallucination. On LiveCodeBench, DuET achieves the state-of-the-art performance, improving Pass@1 by 13.6 pp.

==> table/contribution.tex <==
\begin{table}[tb!]
    \centering
    \small
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{lcccc}
        \thickhline
                                                                    & \textbf{Decoupled}       & \textbf{Grounding} \\
        \hline
        \textsc{CodeT}{\scriptsize~\cite{chen2023codet}}            & \xmark                   & -                  \\
        TestChain{\scriptsize~\cite{li2024largelanguagemodelstest}} & \cmark                   & Code               \\
        \rowcolor{gray!20}
                                                                    &                          & Code \&            \\
        \rowcolor{gray!20}
        \multirow{-2}{*}{\ours {\scriptsize~(this work)}}                         & \multirow{-2}{*}{\cmark} & Pseudocode         \\
        \thickhline
    \end{tabular}
    \caption{
        \ours decouples test input generation and test output prediction, while grounding both code and pseudocode in test output prediction.
    }
    \label{tab:contribution}
\end{table}
